The Superconformal Index of the (2,0) Theory with Defects

We compute the supersymmetric partition function of the six-dimensional $(2,0)$ theory of type $A_{N-1}$ on $S^1 \times S^5$ in the presence of both codimension two and codimension four defects. We concentrate on a limit of the partition function depending on a single parameter. From the allowed supersymmetric configurations of defects we find a precise match with the characters of irreducible modules of $W_N$ algebras and affine Lie algebras of type $A_{N-1}$.

==> Final ArXiv/preamble.tex <==
%-------------------------------------------------------------

\usepackage{amsfonts}
\usepackage{amscd}
\usepackage{amssymb}
\usepackage{amsmath,bbm}
\usepackage{graphicx}
\usepackage{epsfig}
\usepackage{latexsym}
\usepackage{mathtools}
\usepackage{hyperref}
\usepackage[vcentermath]{youngtab}
\hypersetup{
    colorlinks=true,
   linkcolor=black,
    citecolor=black,
    filecolor=black,
    urlcolor=black,}
    
%-------------------------------------------------------------

\newcommand{\pathtodiagrams}{figures/}

\newcommand{\mathfig}[2]{{\hspace{-3pt}\begin{array}{c}%
  \raisebox{-2.5pt}{\includegraphics[width=#1\textwidth]{\pathtodiagrams #2}}%
\end{array}\hspace{-3pt}}}


%--------------------------------------------------------------

\def \be  {\begin{equation}}
\def \ee  {\end{equation}}
\def \bea {\begin{equation}\begin{aligned}}
\def \eea {\end{aligned}\end{equation}}
\def \ba  {\begin{eqnarray}}
\def \ea  {\end{eqnarray}}
\def \bb  {\begin{thebibliography}}
\def \eb  {\end{thebibliography}}
\def \lab #1 {\label{#1}}

%-------------------------------------------------------------

\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cJ{\mathcal{J}}
\newcommand\cK{\mathcal{K}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}
\newcommand\cP{\mathcal{P}}
\newcommand\cQ{\mathcal{Q}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cT{\mathcal{T}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}
\newcommand\cW{\mathcal{W}}
\newcommand\cY{\mathcal{Y}}
\newcommand\cZ{\mathcal{Z}}
\newcommand\al{\alpha}
\newcommand\si{\sigma}
\newcommand\dal{\dot\alpha}
\newcommand\Qbar{\bar{Q}}
\newcommand\rf{*}
\newcommand\U{\Upsilon}
\newcommand\q{\mathfrak{q}}
\newcommand\af{\mathfrak{a}}
\newcommand\tf{\mathfrak{t}}
\newcommand\qf{\mathfrak{q}}
\newcommand\pf{\mathfrak{p}}
\newcommand\xf{\mathfrak{x}}
\newcommand\slf{\mathfrak{sl}}
\newcommand\gf{\mathfrak{g}}
\newcommand\sutwo{\mathfrak{su}(2)}

\newcommand\mr{\mathrm{m}}
\newcommand\bC{\mathbb{C }}
\newcommand\bP{\mathbb{P}}
\newcommand\bQ{\mathbb{Q}}
\newcommand\bR{\mathbb{R}}
\newcommand\bT{\mathbb{T}}
\newcommand\bZ{\mathbb{Z}}

\newcommand\SU{\mathrm{SU}}
\newcommand\rD{\mathrm{D}}
\newcommand\rP{\mathrm{P}}
\newcommand\rU{\mathrm{U}}
\newcommand\rW{\mathrm{W}}
\newcommand\rZ{\mathrm{Z}}
\newcommand\ru{\mathrm{u}}

\newcommand\rd{\mathrm{d}}
\newcommand\e{\mathrm{e}}
\newcommand\im{\mathrm{i}}


\newcommand\lb{\lambda}
\newcommand\tlb{\tilde{\lambda}}
\newcommand\teta{\tilde{\eta}}
\newcommand\la{\langle}
\newcommand\ra{\rangle}
\newcommand\del{\partial}
\newcommand\delbar{\bar{\partial}}
\newcommand\Dbar{\bar{\mathcal{D}}}
\newcommand\tr{\mathrm{Tr}}
\newcommand\SUN{\mbox{SU}(N)}
\newcommand\ir{\mathrm{IR}}
\newcommand\uv{\mathrm{UV}}
\newcommand\ep{\epsilon}

\newcommand\rrangle{\ra\ra}
\newcommand{\PE}[1]{ \mathrm{PE}\left[ #1 \right] }


